Leafy Automata for Higher-Order Concurrency

Finitary Idealized Concurrent Algol (FICA) is a prototypical programming language combining functional, imperative, and concurrent computation. There exists a fully abstract game model of FICA, which in principle can be used to prove equivalence and safety of FICA programs. Unfortunately, the problems are undecidable for the whole language, and only very rudimentary decidable sub-languages are known. We propose leafy automata as a dedicated automata-theoretic formalism for representing the game semantics of FICA. The automata use an infinite alphabet with a tree structure. We show that the game semantics of any FICA term can be represented by traces of a leafy automaton. Conversely, the traces of any leafy automaton can be represented by a FICA term. Because of the close match with FICA, we view leafy automata as a promising starting point for finding decidable subclasses of the language and, more generally, to provide a new perspective on models of higher-order concurrent computation. Moreover, we identify a fragment of FICA that is amenable to verification by translation into a particular class of leafy automata. Using a locality property of the latter class, where communication between levels is restricted and every other level is bounded, we show that their emptiness problem is decidable by reduction to Petri net reachability.

==> lncs-resources/style-guide.tex <==
%
%
%
\section{First Section}
\subsection{A Subsection Sample}
Please note that the first paragraph of a section or subsection is
not indented. The first paragraph that follows a table, figure,
equation etc. does not need an indent, either.

Subsequent paragraphs, however, are indented.

\subsubsection{Sample Heading (Third Level)} Only two levels of
headings should be numbered. Lower level headings remain unnumbered;
they are formatted as run-in headings.

\paragraph{Sample Heading (Fourth Level)}
The contribution should contain no more than four levels of
headings. Table~\ref{tab1} gives a summary of all heading levels.

\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|}
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}


\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}
Please try to avoid rasterized images for line-art diagrams and
schemas. Whenever possible, use vector graphics instead (see
Fig.~\ref{fig1}).

\begin{figure}
\includegraphics[width=\textwidth]{fig1.eps}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig1}
\end{figure}

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}
For citations of references, we prefer the use of square brackets
and consecutive numbers. Citations using labels or the author/year
convention are also acceptable. The following bibliography provides
a sample reference list with entries for journal
articles~\cite{ref_article1}, an LNCS chapter~\cite{ref_lncs1}, a
book~\cite{ref_book1}, proceedings without editors~\cite{ref_proc1},
and a homepage~\cite{ref_url1}. Multiple citations are grouped
\cite{ref_article1,ref_lncs1,ref_book1},
\cite{ref_article1,ref_book1,ref_proc1,ref_url1}.
%
% ---- Bibliography ----
%
% BibTeX users should specify bibliography style 'splncs04'.
% References will then be sorted and formatted in the correct style.
%

==> sections-apx/03-sla-decidable-old.tex <==
\section{Proof of Theorem \ref{thm:sla-decidable}}
\label{apx:sla-decidable}


{
\newcommand{\quu}{\ensuremath{q^{(i-2)}}}
\newcommand{\qu}{\ensuremath{q^{(i-1)}}}
\newcommand{\qi}{\ensuremath{q^{(i)}}}
\newcommand{\qii}{\ensuremath{q^{(i+1)}}}
\newcommand{\qiii}{\ensuremath{q^{(i+2)}}}

\newcommand{\qpuu}{\ensuremath{q^{\prime(i-2)}}}
\newcommand{\qpu}{\ensuremath{q^{\prime(i-1)}}}
\newcommand{\qpi}{\ensuremath{q^{\prime(i)}}}
\newcommand{\qpii}{\ensuremath{q^{\prime(i+1)}}}
\newcommand{\qpiii}{\ensuremath{q^{\prime(i+2)}}}

\newcommand{\mapping}[1]{\ensuremath{\{~#1~\}}}
\renewcommand{\and}{\ensuremath{,~}}

For every even layer $i = k, k-2, ..., 0$, we construct summary sets of the following shape:
\[
S^{(i)}_x = (\alpha, s_1, ..., s_{\leq b}, \omega) \in Q^{(i)} \times (Q^{(i-2, i-1)} \times Q^{(i-2, i-1)})^{\leq 2b} \times Q^{(i)}
\]

\ad{TODO: RLA probably won't appear in the paper so this proof must include all the prelims that were dealt with in the RLA proof.}

where $X^{\leq 2b}$ indicates a sequence of elements of $X$ of length at most $2b$, twice the even layer bound. In words, this indicates that a node at layer $i$ may go from state $\alpha$ to state $\omega$, being child-free at each end, and performing at most $r \leq 2b$ stateful read-writes  $\mathsf{INT}_{x,r}$ of the next even layer up. For simplicity, we will assume that every operation on values above is an atomic read/write.

\paragraph* {Inductive step.} 
Suppose that we have the summary sets at level $i+2$.
We construct a VASS query for every possible combination of
\begin{itemize}
    \item start state $\alpha \in Q^{(i)}$;
    \item end state $\omega \in Q^{(i)}$;
    \item read value $(r, \quu), (r,\qu)$ in each of the $r \in [0,2b]$ possible instances of reading the state above;
    \item write value $(r, \qpuu), (r, \qpu)$ in each of the $r \in [0,2b]$ possible instances of writing to the state above.
    \item integer $u \in [0,b]$ of \emph{used} children.
\end{itemize}

The reachability query asks whether we can, from
\[ 
\left\{
\begin{aligned}
   \forall r \in [0,2u-1] \colon (\mathsf{read}, r, \quu) = 1, (\mathsf{read}, r, \qu) = 1 & \qquad
   \alpha = 1 \\
   \forall j \in [1,b] \colon (j, \bot) = 1 & \qquad
   (c,0) = 1
\end{aligned}
\right\}
\]

all other places zero, reach
\[ 
\left\{
\begin{aligned}
   \forall r \in [0,2u-1] \colon (\mathsf{write}, r, \qpuu) = 1, (\mathsf{write}, r, \qpu) = 1 & \qquad
   \omega = 1 \\
   \forall j \in [1, u] \colon (j, \top) = 1 & \qquad
   \forall j \in [u+1, b] \colon (j, \bot) = 1\\
   (c, 2u) = 1
\end{aligned}
\right\}
\]
all other places zero.

\ad{$(c,2u)$ means the stateful read-write counter is at position $2u$, i.e. $2u$ stateful reads-writes have been performed. This corresponds to creating and destroying $u$ children.}

If the reachability query succeeds, then we add
\[(\alpha, ((\quu_0, \qu_0),(\qpuu_0, \qpu_0)) ... ((\quu_{2u}, \qu_{2u}),(\qpuu_{2u}, \qpu_{2u})) ,\omega)\]
to the summary set at level $i$.

\paragraph{Places.}

The complete set of places required is as follows:

\vspace{3mm}

\textbf{Read/Write simulation}
\begin{itemize}
    \item For each element of $r \in [0,2b]$, we need a gadget representing an atomic read-write, with:
        \begin{itemize}
            \item A place $(\mathsf{read}, r, q^{(i-2)})$ for each state $q \in Q^{(i-2)}$;
            \item A place $(\mathsf{read}, r, q^{(i-1)})$ for each state $q \in Q^{(i-1)}$;
            \item A place $(\mathsf{write}, r, q^{(i-2)})$ for each state $q \in Q^{(i-2)}$;
            \item A place $(\mathsf{write}, r, q^{(i-1)})$ for each state $q \in Q^{(i-1)}$.
        \end{itemize}
    \item We also need a counter gadget with $2b+1$ places $(\mathsf{c}, 0), ..., (\mathsf{c}, 2b)$, which tracks how many of the read-writes have been used.
\end{itemize}

\textbf{Level-$i$ state}
\begin{itemize}
    \item For each element $q^{(i)} \in Q^{(i)}$, we need one state $q^{(i)}$.
\end{itemize}

\textbf{Children}
\begin{itemize}
    \item For each element of $j \in [1,b]$, we need a gadget representing a child of the level-$i$ node, with:
        \begin{itemize}
            \item A place $(j, q^{(i+1)})$ for each element $q^{(i+1)} \in Q^{(i+1)} \cup \{\bot, \top\}$;
            \item A place $(j, q^{(i+2)})$ for each element $q^{(i+2)} \in Q^{(i+2)}$;
            \item A place $(j, \mathsf{INT}_{x,n})$ for each ``interrupt point'' $\mathsf{INT}_{x,n}$ in each summary $S^{(i+2)}_x \in S^{(i+2)}$.
        \end{itemize}
\end{itemize}

The addition of $\bot$ and $\top$ at level $i+1$ ensures that we do not reuse child gadgets.

\paragraph*{Transitions.}

The transition generators are given below.

\textbf{Adding a child at layer $i+1$:}
\[
\frac
{(\quu, \qu, \qi) \xrightarrow{x_Q} (\qpuu, \qpu, \qpi, \qpii) \in \delta_Q \qquad j \in [1,b] \qquad r \in [0,2b-1]}
{\left\{\begin{aligned}
    (\mathsf{read}, r, \quu) \mapsto -1 & \and (\mathsf{write}, r, \qpuu) \mapsto +1 \\
    (\mathsf{read}, r, \qu) \mapsto -1 & \and (\mathsf{write}, r, \qpu) \mapsto +1 \\
    \qi \mapsto -1 & \and \qpi \mapsto +1 \\
    (j, \bot) \mapsto -1 & \and (j,\qpii) \mapsto +1 \\
    (c, r) \mapsto -1 & \and (c, r+1) \mapsto +1
\end{aligned} \right\} \in T}
\]


\textbf{Adding a child at layer $i+2$:}
\[
\frac
{(\qi, \qii) \xrightarrow{x_Q} (\qpi, \qpii, \qpiii) \in \delta_Q \qquad j \in [1,b]}
{\left\{\begin{aligned}
    \qi \mapsto -1 & \and \qpi \mapsto +1 \\
    (j, \qii) \mapsto -1 & \and (j, \qpii) \mapsto +1 \\
    (j, \qpiii) \mapsto +1 
\end{aligned} \right\} \in T}
\]

\textbf{Removing a child at layer $i+1$:}
\[
\frac
{(\quu, \qu, \qi, \qii) \xrightarrow{x_A} (\qpuu, \qpu, \qpi) \in \delta_A \qquad j \in [1,b] \qquad r \in [0,2b-1]}
{\left\{\begin{aligned}
    (\mathsf{read}, r, \quu) \mapsto -1 & \and (\mathsf{write}, r, \qpuu) \mapsto +1 \\
    (\mathsf{read}, r, \qu) \mapsto -1 & \and (\mathsf{write}, r, \qpu) \mapsto +1 \\
    \qi \mapsto -1 & \and \qpi \mapsto +1 \\
    (j, \qii) \mapsto -1 & \and (j,\top) \mapsto +1 \\
    (c, r) \mapsto -1 & \and (c, r+1) \mapsto +1
\end{aligned} \right\} \in T}
\]


\textbf{Removing a child at layer $i+2$:}
\[
\frac
{(\qi, \qii, \qiii) \xrightarrow{x_A} (\qpi, \qpii) \in \delta_A \qquad j \in [1,b]}
{\left\{\begin{aligned}
    \qi \mapsto -1 & \and \qpi \mapsto +1 \\
    (j, \qii) \mapsto -1 & \and (j, \qpii) \mapsto +1 \\
    (j, \qiii) \mapsto -1 
\end{aligned} \right\} \in T}
\]

\textbf{Simulation of children at layer $i+2$:}

\ad{Allow the child to freely move to the first interrupt point:}
\[
\frac
{(\alpha^{(i+2)}, \mathsf{INT}_{x,0},...,\mathsf{INT}_{x,n}, \omega^{(i+2)}) \in S^{(i+2)} 
\qquad j \in [1,b]}
{\left\{\begin{aligned}
    (j, \alpha^{(i+2)}) \mapsto -1 \and (j, \mathsf{INT}_{x,0}) \mapsto +1
\end{aligned} \right\} \in T}
\]

% \[
% \frac
% {(a, \mathsf{INT}_{x,0},...,\mathsf{INT}_{x,n}, b) \in S^{(i+2)} 
% \qquad j \in [1,b]}
% {\left\{\begin{aligned}
%     (j, \mathsf{INT}_{x,n}) \mapsto +1 \and (j, b) \mapsto +1
% \end{aligned} \right\} \in T}
% \]

\ad{Perform an interrupt then freely move to the next one:}
\[
\frac
{(\alpha^{(i+2)}, \mathsf{INT}_{x,0},...,\mathsf{INT}_{x,n}, \omega^{(i+2)}) \in S^{(i+2)} 
\qquad r \in [0, n-1]
\qquad ((\qi, \qii), (\qpi, \qpii)) = \mathsf{INT}_{x,r}
\qquad j \in [1,b]}
{\left\{\begin{aligned}
    \qi \mapsto -1 & \and \qpi \mapsto +1 \\
    (j,\qii) \mapsto -1 & \and (j,\qpii) \mapsto +1 \\
    (j, \mathsf{INT}_{x,r}) \mapsto -1 & \and (j, \mathsf{INT}_{x,r+1}) \mapsto +1
\end{aligned} \right\} \in T}
\]


\ad{Perform the final interrupt:}
\[
\frac
{(\alpha^{(i+2)}, \mathsf{INT}_{x,0},...,\mathsf{INT}_{x,n}, \omega^{(i+2)}) \in S^{(i+2)} 
\qquad ((\qi, \qii), (\qpi, \qpii)) = \mathsf{INT}_{x,n}
\qquad j \in [1,b]}
{\left\{\begin{aligned}
    \qi \mapsto -1 & \and \qpi \mapsto +1 \\
    (j,\qii) \mapsto -1 & \and (j,\qpii) \mapsto +1 \\
    (j, \mathsf{INT}_{x,r}) \mapsto -1 & \and (j, \omega^{(i+2)}) \mapsto +1
\end{aligned} \right\} \in T}
\]


\paragraph* {Base case.}
The base case is $i=k$ for even $k$, or $i=k-1$ for odd $k$. This is the same as the inductive case, except there are no nodes at layer $k+2$ so the VASS construction is slightly easier. No special tricks are needed.

\paragraph* {Level 0.}
Level 0 can be handled the same as any other level, but there will be no read-writes above so elements of the summary set will be in $Q^{(0,0)}$. In order to use the same inductive mechanism we can pretend that $Q^{(-1)} = Q^{(-2)} = \{\bot\}$.

}

==> sections-apx/03-sla-decidable.tex <==
\section{Additional material for Section~\ref{sec:lla}}

\subsection{Proof of Theorem \ref{thm:sla-decidable}}
\label{apx:sla-decidable}

{

% Some local definitions used in this proof!

\newcommand{\quu}{\ensuremath{q^{(2i-2)}}}
\newcommand{\qu}{\ensuremath{q^{(2i-1)}}}
\newcommand{\qi}{\ensuremath{q^{(2i)}}}
\newcommand{\qii}{\ensuremath{q^{(2i+1)}}}
\newcommand{\qiii}{\ensuremath{q^{(2i+2)}}}

\newcommand{\qpuu}{\ensuremath{q^{\prime(2i-2)}}}
\newcommand{\qpu}{\ensuremath{q^{\prime(2i-1)}}}
\newcommand{\qpi}{\ensuremath{q^{\prime(2i)}}}
\newcommand{\qpii}{\ensuremath{q^{\prime(2i+1)}}}
\newcommand{\qpiii}{\ensuremath{q^{\prime(2i+2)}}}

\renewcommand{\interrupt}{\mathsf{interrupt}}
\renewcommand{\read}{\mathsf{read}}
\renewcommand{\write}{\mathsf{write}}
\newcommand{\state}{\mathsf{state}}
\newcommand{\child}{\mathsf{child}}
\newcommand{\grandchildren}{\mathsf{grandchildren}}
\renewcommand{\r}{\mathsf{r}}

\newcommand{\mapping}[1]{\ensuremath{\{~#1~\}}}
\renewcommand{\and}{\ensuremath{,~}}

\makeatletter
\newcommand{\alist}[1]{%
    \begin{aligned}[t] & #1\checknextarg}
\newcommand{\checknextarg}{\@ifnextchar\bgroup{\gobblenextarg}{ \end{aligned} }}
\newcommand{\gobblenextarg}[1]{ \\ & #1\@ifnextchar\bgroup{\gobblenextarg}{ \end{aligned} }}
\makeatother

\newcommand{\vassrule}[3]{
\[
\begin{aligned}
\textbf{for all}~~ & #1 \\
\textbf{if}~~ & #2 \\
\textbf{then}~~ & #3
\end{aligned}
\]
}

We continue from the proof sketch described that accompanies Theorem \ref{thm:sla-decidable}. Recall that we intend to inductively construct summaries at level $2i$, given summaries at level $2i+2$, by reduction to VASS reachability.


Let us define the \emph{candidate set} $C^{(2i)}$ for layer $2i$ as follows:

\[
C^{(2i)} = Q^{(2i)} \times (Q^{(2i-2, 2i-1)} \times Q^{(2i-2, 2i-1)})^{\leq 2b} \times Q^{(2i)}
\]

A candidate $c = (\alpha^{(2i)}, \mathsf{INT}_1, \cdots, \mathsf{INT}_m, \omega^{(2i)})$ is a \emph{summary} at level $2i$ if and only if some series of transitions exists such that a node at level $2i$ may go from state $\alpha^{(2i)}$ without any children to state $\omega^{(2i)}$ without any children, and in between performing read-write accesses $\mathsf{INT}_n$ in order. We naturally define the \emph{summary set} $S^{(2i)} \subseteq C^{(2i)}$ as the subset of the candidate set such that every element is a summary at level $2i$. 

Constructing the summary set for the deepest layer ($2i = k$) is simple: nodes on the bottom-most level may spawn no children by definition and so they have no opportunity to change state, ergo the summary set is the identity function on $Q^{(k)}$: $S^{(k)} = \{~(q,q) ~|~ q \in Q^{(k)}~\}$.

Assume that we have the complete summary set $S^{(2i+2)}$ for level $2i+2$. We shall compute the summary set $S^{(2i)}$ for level $2i$.

Enumerating the whole candidate set is simple, as every component is bounded. For each candidate $s = (\alpha, \interrupt(s,0), \cdots, \interrupt(s,m), \omega)$, with $m$ interrupt points, we test whether or not it is a summary at level $2i$ in the following~way.

For convenience, let us define $\interrupt(s, r) = ((\quu, \qu), (\qpuu, \qpu))$ as the read-write pair in the $r$th interrupt of the candidate $s$ that we are testing. We also define $\read(s,r) = (\quu, \qu)$ and $\write(s,r) = (\qpuu, \qpu)$.

The procedure for determining whether a candidate $s$ is a valid summary is represented here by a nondeterministic program over finite variables and unbounded counters (without zero tests). The program is a set of rules which will be nondeterministically evaluated. Either some run of the program will complete and \texttt{ACCEPT}, or all paths will block with no more rules that can be applied. Such programs are known to be reducible to VASS reachability. 

The variables of the program are:
\[
\r \in [0,2b] \qquad 
\state \in Q^{(2i)} \qquad 
\child[j] \in Q^{(2i+1)} \cup \{\bot,\top\}
\]

and the unbounded counters are: 
\[
   \grandchildren[j,s,p] \in \mathbb{N}
\]

such that:
\begin{itemize}
    \item $\r$ captures the number of reads-writes performed so far in the evaluation.
    \item $\state$ captures the state of our level $2i$ node.
    \item $\child[j]$ (where $j \in [1,b]$) captures the state of the (at most $b$) children at level $2i+1$. We include additional states $\{\bot, \top\}$ to represent children which have not yet been created, and children which have since been destroyed, respectively.
    \item $\grandchildren[j,s,p]$ (where $j \in [1,b]$, $s \in S^{(2i+2)}$, $p \in [0,m]$) are counters for every combination of child, level $2i+2$ summary, and interrupt point along that summary. Note that $j$ also includes zero, to represent that no interrupts have yet been performed.
\end{itemize}

The initial values are:
\[
    \r = 0 \qquad 
    \state = \alpha 
    \qquad \forall j \colon \child[j] = \bot
    \qquad  \forall j,s,p \colon \grandchildren[j,s,p] = 0
\]

The rules of the program are as follows. When we write $\textbf{for all}$, one rule is created for every possible assignment of the free variables.

\vspace{5mm}

{
\noindent \textbf{Adding a child.} We first ensure that there is an unused child, and then proceed to populate that child with a state. The precise shape of these additions is dictated by $\delta_Q^{(2i+1)}$.  Note that this rule is predicated on the values of $\interrupt(s,r)$ in the summary.

\vassrule
    {\alist
        {j \in [1,b]}
        {(\read(s,r), \qi) \xrightarrow{x_\Q} (\write(s,r), \qpi, \qpii) \in \delta_\Q^{(2i+1)} }
    }
    {\alist
        {\state      = \qi}
        {\child[j]   = \bot}
    }
    {\alist
        {\state = \qpi}
        {\child[j] = \qpii}
        {\r = \r + 1}
    }
    
}

{
\noindent \textbf{Removing a child.} We move a child at level $2i+1$ into the top state to show that it has been removed. No further operations on grandchildren are permitted.

\vassrule
    {\alist
        {j \in [1,b]}
        {(\read(s,r), \qi, \qii) \xrightarrow{x_\A} (\write(s,r), \qpi) \in \delta_\A^{(2i+1)} }
    }
    {\alist
        {\state      = \qi}
        {\child[j]   = \qii}
    }
    {\alist
        {\state = \qpi}
        {\child[j] = \top}
        {\r += 1}
    }
    
}

{
\noindent \textbf{Adding a grandchild.} We add a new leaf as the child of a currently active child. We choose a summary for the node to follow and indicate that it is yet to make any interrupts.

\vassrule
    {\alist
        {j \in [1,b]}
        {(\qi, \qii) \xrightarrow{x_\Q} (\qpi, \qpii, \qpiii) \in \delta_\Q^{(2i+2)} }
        {s^{(2i+2)} = (\qpiii, \cdots) \in S^{(2i+2)}}
    }
    {\alist
        {\state      = \qi}
        {\child[j]   = \qii}
    }
    {\alist
        {\state      = \qpi}
        {\child[j]   = \qpii}
        {\child[j,s^{(2i+2)},0] \text{ += } 1}
    }
    
}

{
\noindent \textbf{Removing a grandchild.} We may remove a grandchild at level $2i+2$ once it has progressed through all interrupt points (hence reached a new child-free state $\qpiii$. The shape of these additions is dictated by $\delta_A^{(2i+2)}$.

\vassrule
    {\alist
        {j \in [1,b]}
        {(\qi, \qii, \qiii) \xrightarrow{x_\A} (\qpi, \qpii) \in \delta_\A^{(2i+2)} }
        {s^{(2i+2)} = (\cdots, \interrupt(s^{(2i+2)},m), \qiii) \in S^{(2i+2)}}
    }
    {\alist
        {\state      = \qi}
        {\child[j]   = \qii}
        {\grandchildren[j, s^{(2i+2)}, m] \geq 1}
    }
    {\alist
        {\state      = \qpi}
        {\child[j]   = \qpii}
        {\grandchildren[j, s^{(2i+2)}, m] \text{ -= } 1}
    }
}

{
\noindent \textbf{Progressing a grandchild.} Grandchildren may progress at any time, so long as the current state of our top-level node and the intermediate child align with the read values of the next interrupt in the summary that it is following. 

\vassrule
    {\alist
        {j \in [1,b]}
        {n \in [0,2b-1]}
        {s^{(2i+2)} = (\cdots, \interrupt(s^{(2i+2)},n), \cdots) \in S^{(2i+2)}}
        {(\qi, \qii),(\qpi, \qpii) = \interrupt(s^{(2i+2)},n)}
    }
    {\alist
        {\state      = \qi}
        {\child[j]   = \qii}
        {\grandchildren[j, s^{(2i+2)}, n] \geq 1}
    }
    {\alist
        {\state      := \qpi}
        {\child[j]   := \qpii}
        {\grandchildren[j, s^{(2i+2)}, n] \text{ -= } 1}
        {\grandchildren[j, s^{(2i+2)}, n+1] \text{ += } 1}
    }
}

The program will \texttt{ACCEPT} if it reaches the following configuration:
\[
    \r = m \qquad 
    \state = \omega 
    \qquad \forall j \colon \child[j] = \top
    \qquad  \forall j,s,p \colon \grandchildren[j,s,p] = 0
\]
Hence we have reached the end state $\omega$; all $m$ interrupts have been performed; all children have been used; and no grandchildren remain. 

The translation of the above system of instructions to VASS is short: the current state is the product of all the program variables, and the vector components are the $\grandchildren$ counters. The rules exactly correspond to transitions, with omitted variables permitting any value. 


}
